Learning to Link

Clustering is an important part of many modern data analysis pipelines, including network analysis and data retrieval. There are many different clustering algorithms developed by various communities, and it is often not clear which algorithm will give the best performance on a specific clustering task. Similarly, we often have multiple ways to measure distances between data points, and the best clustering performance might require a non-trivial combination of those metrics. In this work, we study data-driven algorithm selection and metric learning for clustering problems, where the goal is to simultaneously learn the best algorithm and metric for a specific application. The family of clustering algorithms we consider is parameterized linkage based procedures that includes single and complete linkage. The family of distance functions we learn over are convex combinations of base distance functions. We design efficient learning algorithms which receive samples from an application-specific distribution over clustering instances and simultaneously learn both a near-optimal distance and clustering algorithm from these classes. We also carry out a comprehensive empirical evaluation of our techniques showing that they can lead to significantly improved clustering performance.

==> omniglot-experiments.tex <==
\subsection{Clustering Subsets of Omniglot}

\paragraph{Problem Formulation.} The omniglot dataset contains images of handwritten characters from 30 different alphabets that include well-known ones such as Latin and Greek and less-known ones such as Gujarati and Tangalog. Each character is represented by 20 drawings from different people as well as the stroke data that indicites the drawings' timings, i.e. the pixel's xy-coordinates matched with a corresponding timestamp.

\paragraph{Intra-Alphabet Experiments.} First, we started looking at all the 30 alphabets individually where each of them has between 14 and 55 different characters. After running this setup with both clustering families, we noticed that there is a huge variety between different alphabets, i.e. we were able to cluster alphabets quite well individually but averaging over all alphabets does not improve the quality much.

\begin{figure}[h]
\centering
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/Cyrillic}
\end{minipage}
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/Inuktitut}
\end{minipage}
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/Ojibwe}
\end{minipage}
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/omniglot-ac-average}
\end{minipage}
\caption{Different alphabets of the omniglot dataset can be clustered well, but in comparison the optimal parameter varies a lot.}
\label{fig:omniglotintraac}
\end{figure}

Figure \ref{fig:omniglotintraac} shows that we get improvements of more than $5\%$ for some of the 30 alphabets, but in average there is no good value $\alpha_{opt}$ that gives major improvements over complete linkage. 

\paragraph{Inter-Alphabet Experiments.} In addition, we tried to cluster characters taken from different alphabets. In our setting, we selected one character from each alphabet randomly and ran multiple repetitions of this setting where each run contains 30 classes, i.e. 600 points. One advantage of this setting is that each run has the same amount of target cluster that made it easier to average the results over all experiments.

\begin{figure}[h]
\centering
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{plots/omniglot-sc-average-inter}
\end{minipage}
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{plots/omniglot-ac-average-inter}
\end{minipage}
\caption{Clustering character of different alphabets only gives a small improvement for using the $\alpha$-linkage algorithm.}
\label{fig:omniglotinter}
\end{figure}

Figure \ref{fig:omniglotinter} shows that also for clustering characters of different alphabets the improvements are rather small. Averaged over 250 runs the improvement shown above was $1.0\%$. In conclusion, the $\alpha$-linkage algorithm did very well for pixel data in situations where we clustered the images within different alphabets, but for both averaging over different alphabets and selecting characters from different alphabets we did not get major improvements.

\paragraph{Experiments with learned features.} Similar to the earlier discussed MNIST experiments, we also tried to apply a learned feature representation to the images prior to the clustering. Therefor, we reused the CNN trained on the MNIST images, because both datasets contain handwritten characters and it seems natural that letters and digits have similar attributes. After generating the feature representations for all Omniglot alphabets, we were running the intra alphabet experiments again and compared the results to the ones where we clustered the raw pixel data. Figure \ref{fig:omniglotmnistfeatures} shows the comparison of using neural network and pixel features for one exemplary alphabet.

\begin{figure}[h]
\centering
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{plots/greek_sc}
\end{minipage}
\begin{minipage}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{plots/greek_sc_mnist}
\end{minipage}
\caption{Using features learned on the MNIST dataset gives major improvements for clustering the Omniglot alphabets. The Greek alphabet demonstrates these improvements.}
\label{fig:omniglotmnistfeatures}
\end{figure}

\todo{experiments using stroke data}
